Disentangled Causal Graph Learning for Online Unsupervised Root Cause Analysis

The task of root cause analysis (RCA) is to identify the root causes of system faults/failures by analyzing system monitoring data. Efficient RCA can greatly accelerate system failure recovery and mitigate system damages or financial losses. However, previous research has mostly focused on developing offline RCA algorithms, which often require manually initiating the RCA process, a significant amount of time and data to train a robust model, and then being retrained from scratch for a new system fault. In this paper, we propose CORAL, a novel online RCA framework that can automatically trigger the RCA process and incrementally update the RCA model. CORAL consists of Trigger Point Detection, Incremental Disentangled Causal Graph Learning, and Network Propagation-based Root Cause Localization. The Trigger Point Detection component aims to detect system state transitions automatically and in near-real-time. To achieve this, we develop an online trigger point detection approach based on multivariate singular spectrum analysis and cumulative sum statistics. To efficiently update the RCA model, we propose an incremental disentangled causal graph learning approach to decouple the state-invariant and state-dependent information. After that, CORAL applies a random walk with restarts to the updated causal graph to accurately identify root causes. The online RCA process terminates when the causal graph and the generated root cause list converge. Extensive experiments on three real-world datasets with case studies demonstrate the effectiveness and superiority of the proposed framework.

==> table/overall_performance.tex <==
\begin{table*}[!ht]
\renewcommand\arraystretch{1}
\centering
	\caption{Overall performance {\it w.r.t.} AIOps, Swat, and WADI datasets.} 
	\vspace{-0.3cm}
\begin{tabular}{c|cccc|cccc|cccc}
\hline
                               & \multicolumn{4}{c|}{AIOps}                                                                                                               & \multicolumn{4}{c|}{Swat}                                                                                                                & \multicolumn{4}{c}{WADI}                                                                                                                 \\ \hline
                               & \multicolumn{1}{c|}{PR@1}             & \multicolumn{1}{c|}{PR@10}            & \multicolumn{1}{c|}{MAP@10}           & MRR              & \multicolumn{1}{c|}{PR@1}             & \multicolumn{1}{c|}{PR@10}            & \multicolumn{1}{c|}{MAP@10}           & MRR              & \multicolumn{1}{c|}{PR@1}             & \multicolumn{1}{c|}{PR@10}            & \multicolumn{1}{c|}{MAP@10}           & MRR              \\ \hline
\textbf{\textbf{\model}} & \multicolumn{1}{c|}{\textbf{80.00\%}} & \multicolumn{1}{c|}{\textbf{100.0\%}} & \multicolumn{1}{c|}{\textbf{98.00\%}} & \textbf{90.00\%} & \multicolumn{1}{c|}{6.25\%}           & \multicolumn{1}{c|}{\textbf{92.71\%}} & \multicolumn{1}{c|}{\textbf{53.96\%}} & 31.72\%          & \multicolumn{1}{c|}{\textbf{35.71\%}} & \multicolumn{1}{c|}{\textbf{83.33\%}} & \multicolumn{1}{c|}{\textbf{56.00\%}} & \textbf{51.90\%} \\ \hline
NOTEARS                        & \multicolumn{1}{c|}{0.0\%}            & \multicolumn{1}{c|}{60.00\%}          & \multicolumn{1}{c|}{44.00\%}          & 20.46\%          & \multicolumn{1}{c|}{6.25\%}           & \multicolumn{1}{c|}{47.92\%}          & \multicolumn{1}{c|}{25.00\%}          & 22.36\%          & \multicolumn{1}{c|}{7.14\%}           & \multicolumn{1}{c|}{41.67\%}          & \multicolumn{1}{c|}{30.80\%}          & 30.12\%          \\ \hline
GOLEM                          & \multicolumn{1}{c|}{20.00\%}          & \multicolumn{1}{c|}{60.00\%}          & \multicolumn{1}{c|}{54.00\%}          & 37.74\%          & \multicolumn{1}{c|}{\textbf{18.75\%}} & \multicolumn{1}{c|}{62.50\%}          & \multicolumn{1}{c|}{33.44\%}          & 30.42\%          & \multicolumn{1}{c|}{7.14\%}           & \multicolumn{1}{c|}{64.29\%}          & \multicolumn{1}{c|}{38.05\%}          & 25.89\%          \\ \hline
Dynotears                      & \multicolumn{1}{c|}{40.00\%}          & \multicolumn{1}{c|}{60.00\%}          & \multicolumn{1}{c|}{58.00\%}          & 50.77\%          & \multicolumn{1}{c|}{\textbf{18.75\%}} & \multicolumn{1}{c|}{58.33\%}          & \multicolumn{1}{c|}{37.08\%}          & \textbf{33.99\%} & \multicolumn{1}{c|}{14.29\%}          & \multicolumn{1}{c|}{46.43\%}          & \multicolumn{1}{c|}{33.76\%}          & 34.28\%          \\ \hline
PC                             & \multicolumn{1}{c|}{20.00\%}          & \multicolumn{1}{c|}{60.00\%}          & \multicolumn{1}{c|}{30.00\%}          & 25.36\%          & \multicolumn{1}{c|}{12.50\%}          & \multicolumn{1}{c|}{53.13\%}          & \multicolumn{1}{c|}{37.40\%}          & 32.27\%          & \multicolumn{1}{c|}{14.29\%}          & \multicolumn{1}{c|}{57.14\%}          & \multicolumn{1}{c|}{35.71\%}          & 30.74\%          \\ \hline
C-LSTM                         & \multicolumn{1}{c|}{0.00\%}           & \multicolumn{1}{c|}{60.00\%}          & \multicolumn{1}{c|}{48.00\%}          & 24.73\%          & \multicolumn{1}{c|}{12.50\%}          & \multicolumn{1}{c|}{60.42\%}          & \multicolumn{1}{c|}{34.17\%}          & 32.86\%          & \multicolumn{1}{c|}{12.50\%}          & \multicolumn{1}{c|}{64.29\%}          & \multicolumn{1}{c|}{42.62\%}          & 33.28\%          \\ \hline
NOTEARS*                       & \multicolumn{1}{c|}{40.00\%}          & \multicolumn{1}{c|}{80.00\%}          & \multicolumn{1}{c|}{76.00\%}          & 60.00\%          & \multicolumn{1}{c|}{6.25\%}           & \multicolumn{1}{c|}{67.71\%}          & \multicolumn{1}{c|}{42.19\%}          & 26.30\%          & \multicolumn{1}{c|}{14.29\%}          & \multicolumn{1}{c|}{72.62\%}          & \multicolumn{1}{c|}{48.38\%}          & 37.74\%          \\ \hline
GOLEM*                         & \multicolumn{1}{c|}{60.00\%}          & \multicolumn{1}{c|}{80.00\%}          & \multicolumn{1}{c|}{78.00\%}          & 70.00\%          & \multicolumn{1}{c|}{6.25\%}           & \multicolumn{1}{c|}{68.75\%}          & \multicolumn{1}{c|}{43.65\%}          & 28.09\%          & \multicolumn{1}{c|}{21.43\%}          & \multicolumn{1}{c|}{73.81\%}          & \multicolumn{1}{c|}{48.98\%}          & 40.24\%          \\ \hline
\end{tabular}
\end{table*}
